Coding for the unsourced A-channel with erasures: the linked loop code

The A-channel is a noiseless multiple access channel in which users simultaneously transmit Q-ary symbols and the receiver observes the set of transmitted symbols, but not their multiplicities. An A-channel is said to be unsourced if, additionally, users transmissions are encoded across time using a common codebook and decoding of the transmitted messages is done without regard to the identities of the active users. An interesting variant of the unsourced A-channel is the unsourced A-channel with erasures (UACE), in which transmitted symbols are erased with a given independent and identically distributed probability. In this paper, we focus on designing a code that enables a list of transmitted codewords to be recovered despite the erasures of some of the transmitted symbols. To this end, we propose the linked-loop code (LLC), which uses parity bits to link each symbol to the previous M symbols in a tail-biting manner, i.e., the first symbols of the transmission are linked to the last ones. The decoding process occurs in two phases: the first phase decodes the codewords that do not suffer from any erasures, and the second phase attempts to recover the erased symbols using the available parities. We compare the performance of the LLC over the UACE with other codes in the literature and argue for the effectiveness of the construction. Our motivation for studying the UACE comes from its relevance in machine-type communication and coded compressed sensing.

==> channel_model.tex <==

\section{Channel Model}
\label{sec:Channel Model}

The UACE is a variation of the unsoured A-channel from \cite{lancho2022finite} that also encompasses symbol erasures.
%
%These erasures 
%
%Very briefly, 
In the (perfect) unsourced A-channel of \cite{lancho2022finite}, the channel output corresponding to the $l^{\rm th}$ channel use is defined as 
\ea{
\textstyle Y(l) = \bigcup_{k \in [K]} x_{k}(l),
\label{eq:channel perfect}
}
where $x_{k}(l) \in \Qcal$.
%
When transmission takes place over $L$ channel uses,  
we indicate the $L$ channel outputs as $\Yv=[ {Y}(0),\ldots,Y({L-1})]$ .
%for $l \in [L]$.   
%
The $L$ channel inputs corresponding to user $k$ are labeled as $\xv_k=[ x_{k}(0),\ldots,x_{k}(L-1) ]$.  
%
%To indicate the set of outputs $\{Y_t\}_{t \in [T]}$ we use the vector notation $\Yv$.

The UACE is the variation of the model in \eqref{eq:channel perfect} defined in \eqref{eq:channel error}. 
%has already been defined in \eqref{eq:channel error}.
%
Note that $|Y(l)|$ is a random variable which may be less than $K$ due to both collisions and erasures. 
Here, a collision refers to the event when two distinct users $i\neq j$ share a same symbol $x_{i}(l)=x_{j}(l) \in \Qcal$.
%
% \sr{what else we add?}
%
Note that the UACE in \eqref{eq:channel error} is parametrized by the number of users $K$, the cardinality of the input set $Q$, and the erasure probability $p_e$. 
%
%\sr{it might be better to use lower case letters for input and output. upper case for constants. less confusing.}
%
%\sr{}
%

\subsection{Binary Vector Representation}
\label{sec:Binary representation}

%Generally speaking, it is more convenient to consider the case in which $Q=2^J$ for some $J \in \Nbb$, so that one can more conveniently describe the transmission of bits.
%
%In the following, we shall use the underline notation to identify 
%
%In the following sections we shall  describe coding for the UACE whi  $\rb{GF}_2$ for 
When describing coding schemes, it is often convenient to operate over a field; this is also the case also for the UACE.
%
For this reason, we introduce a specific notation for the case in which $Q=2^J$ for some $J \in \Nbb$. 
%
% For this case we let $\Qcal = [2]^J$ and the let the binary vector representation of the UACE 
Let $x_{k}(l)$ be denoted by a $J$-bit binary vector $\vv_{k}(l)$. 
%the binary equivalent of the formulation 
Then, the channel output may be expressed as
% \ea{
% \underbrace{\bold{v}_k(l)}_{\text{\wz{I use the same notation as in URA CCS BP}}} \coloneqq \xu_{l,k} \in [2]^{J}, 
% }where $\xu_{l,k}$ is the binary expression of $x_{l,k}$ in $J$ bits. So that 
\ea{
\textstyle \yv(l) = \bigcup_{k \in [K]}  \delta_{E_{lk}} \lb \bold{v}_{k}(l) \rb.
}
%where $\yv_{l} \in \mathbb{F}_2^J$.
After $L$ uses of the channel, what we obtain may be expressed as the tuple 
\ea{
\Yv =\lsb \yv(0),\yv(1), \ldots ,\yv({L-1})\rsb.
}
%
Moving forward, it shall be convenient to represent the concatenation of the $L$ input binary vectors, each comprised of $J$ bits, as a single row vector; that is
% Again, due to erasure, as well as collision, $|Y_l|\leq K, \forall l \in [L]$. And $\bold{v}_k$ is defined using concatenation as 
\ea{
\bold{v}_k = \bold{v}_k(0).\bold{v}_k(1) \ldots \bold{v}_k(L-1).
\label{eq:input binary size N}
}
%
In this case, we have that the binary representation of the input of user $k$ is  a binary vector $\vv_k$ of dimension $N=JL$.

% SR2WZ: double check again pls
%\textcolor{red}{We have switched indexing notations from $\vv_{l, k}$ to $\vv_k(l)$. We should a standard notation throughout.}
%
% %We denote this set of outputs as $\yvu$. 
% \sr{complete}





% \vspace{1cm}
%
% \sr{do we need a notation for the binary inputs?}
% 
% \subsection{Perfect Unsourced A-channel}
%
% Let the (perfect) unsourced A-channel be defined as follows.
% $K$ users in transmit symbols from a $Q$-ary input alphabet $[Q]$ over a MAC channel with input/output relationship at time $t \in [T]$ is defined as 
% \ea{
% Y_t = \bigcup_{k \in [K]} X_{lk},
% \label{eq:channel perfect}
% }
% where $x_{lk} \in [Q]$
% To indicate the set of outputs $\{Y_t\}_{t \in [T]}$ we use the vector notation $\Yv$.
% %

% \subsection{A-channel with Errors}
% The first variation in the perfect model is the one in which the list size is unchanged, i.e. $K$, but entries are corrupted at random with probability $p_e$.
% %
% In this channel model, then, the channel output is obtained as 
% \ea{
% Y_t = \bigcup_{k \in [K]} \lb X_{lk} E_{lk} + (1-E_{lk}) E_{lk} \rb,
% \label{eq:channel error}
% }
% where $E_{lk} \sim \Bcal(p_e)$ and $E_{lk} \in \Ucal([Q])$ iid for each $t\in T$ and $k \in K$.


% \subsection{A-channel with Insertions and Deletions }
% Next, we are concerned with the 
% \ea{
% Y_t = \bigcup_{k \in [K]} \lb E_{lk} X_{lk}+ (1-E_{lk}) \emptyset  \rb+  \bigcup_{q \in [Q]} q I_{tq}
% \label{eq:channel insertion erasure}
% }
% where $E_{lk} \sim \Bcal(p_e)$ and $I_{lk} \sim \Bcal(p_i)$ iid for each $t\in T$ and $k \in K$.


% \vspace{1cm}
% \sr{2WZ: add table of symbols}


\subsection{Coding for the UACE}

%Next, let us introduce a series of rather standard definitions for coding over a UACE.
%
Let us consider the problem in which each user $k\in [K]$ wishes to transmit a payload of $B$ bits within $L$ channel uses. 
%
Assume payload $\Wv=\{\wv_k\}_{k \in [K]}$ is drawn uniformly at random from $[2]^B$. 
%
Let us refer to $\wv \in \Wv$ as an \emph{active} payload, whereas $[2]^B \setminus \Wv$ contains \emph{inactive} payloads.
%
Finally, if two users randomly select the same payload, let us refer to this event as a payload \emph{collision}.
\begin{definition}[$(L,B)$ Code]
\label{def:code}
A code of block-length $L$ and payload length $B$ for the UACE with parameters $(K,Q,p_e)$ is defined as a (possibly) random \emph{encoding} mapping to produce $L$ channel inputs at each user $k \in [K]$ to encode their message $\wv_k$, defined as
\ea{
%\underbrace{\vv_k}_{\in [2]^N} =  f_{\rm enc} (\underbrace{\wv_k}_{\in [2]^B}),
\xv_k = f_{\rm enc} \lb  \wv_k \rb, 
\label{eq:encoding fun}
}
where $\wv_k \in [2]^B$ and $\xv_k \in \Qcal^L$,
together with a (possibly) random \emph{decoding} mapping which produces a list of transmitted payloads from the channel output, that is
%of active payloads $\widehat{W}(\yv)$, the output of the decoding function given the received $\yv$ of the UACE.
\ea{
\Whv = 
% \lcb \wh_k\rcb_{k \in [K]} = 
f_{\rm dec}( \Yv),
\label{eq:decoding fun}
}
with  $|\Whv|=\Kh$.
% \wz{I think should be: with $K' \coloneqq |\widehat{\bold{W}}|.$}
%\leq K$.
\end{definition}
In other words, the encoding function maps the $B$-bit message $\wv_k$ into the $L$-tuple of channel inputs $\xv_k$. 
%
Upon observing the $L$ channel outputs, $\Yv$, the decoding function produces a list of payloads that are likely to be active. 
%comprise the channel output. 
%
%In the following, we refer to a payload transmitted by at least one user as \underline{active}, while a payload that is not transmitted by any of the users as \underline{inactive}.
%
The list of possibly active payloads produced by the decoding function has length $\Kh$. 
%
%Since the actual number of users is $K$, $K'< K$ indicates the possibility that (i) two users chose the same payload - an event that we define as a \emph{collision}, or (ii) the pattern of erasures is such that the payload of some users cannot be recovered from the channel output. 
%
%
% The size of the output set is contrained can cannot exceed $K$, i.e., $|\widehat{W}(\yv)| \leq K$.
%
Note that the rate of the code in Def.~\ref{def:code} is obtained as $R = B/L$. 
%
Also note that in a UACE each encoder $k \in [K]$ utilizes the same encoding function, so that the identity of the transmitter remains immaterial. 
%: this is in contrast with the classic A-channel or the multiple access channel, in which each user utilizes  a different encoding function. 
%
% \sr{say up to a permutation}
%
\begin{definition}[Payload Probability of Error]
\label{def:pupe}
%
Given code with parameters $(N,B)$ for a UACE with parameters $(K,Q,p_e)$, define 
\begin{itemize}[nolistsep,leftmargin=*]
    \item the Payload Dropping Probability (PDP) as
    \ea{
P_{\rm PDP} = \f 1 K  \sum_{k \in [K]} \Pr \lsb \wv_k \not \in \Whv(\Yv) | \wv_k \in \Wv \rsb,
%
\label{eq:PDP}
}
    \item the Payload Hallucination Probability (PHP) as
\ea{
P_{\rm PHP} = \f 1 {\Kh}  \sum_{k' \in [\Kh]} \Pr \lsb  \wv_{k'} \not \in \Wv | \wv_{k'}  \in \Whv(\Yv) \rsb,
%
\label{eq:PHP}
}    
\end{itemize}
%
% the PUPE is defined as 
% \ea{
% P_e = \f 1 K  \sum_{k \in [K]} \Pr \lsb \wv_k \not \in \widehat{W}(\yv) \rsb,
% %
% \label{eq:PUPE}
% }
where the probability in \eqref{eq:PDP} and \eqref{eq:PHP} is taken over (i) 
%\wz{What does this (i) mean?} 
% it's just a way to list things, just techincal english
the choice of the payload at each user which is selected uniformly at random over $[2]^B$,  (ii) the realization of the erasure sequence, and (iii) the possible randomness in the encoding and decoding functions. 
\end{definition}

More informally, the PDP indicates the probability that a payload is declared inactive when it was actually active, while the PHP indicates the probability that a payload is declared active when it was indeed inactive. 
%
The PDP and PHP are somewhat analogous to the type I and type II errors, respectively, in the hypothesis testing literature.  

% \vspace{1cm}
% \sr{3/3 got here}
% \vspace{1cm}

% \sr{add discussion collisions, say we consider the probability is always vanishing}

% \vspace{1cm}
% \sr{need to change the definition to include false alarms?}

% Note that, in Def. \ref{def:code}, the decoder always outputs $K$ estimates of the active payloads. 
% %
% This constraints simplifies the definition of a transmission error in Def. \ref{eq:pupe}: if $ w_k \not \in \whv$, then there exists a non active payload in $\whv$. 
% %
% A more refined error analysis would consider a decoder that outputs  $K' \leq K$ list of transmitted codewords, so that two error events would be considered: (i) an active payload declared as non active, and (ii) a non-active payload declared as active. 
% %
% %
% %since  does not consider the false alarm event, that is does not allow the decoder  
%
%\vspace{3cm}
% %
% \begin{remark}{\bf Birthday problem}
% Payload collision is analogous to the classic birthday problem,  that is the probability of a collision is similar to the probability that two people in a certain group share the same birthday. 
% %\sr{say we assume no two paylodas are the same}
% In the parameter regimes which we investigate, the probability of payload collision is orders of magnitude smaller that the PDP and PHP of Def. \ref{def:pupe}.
% For this reason, we generally do not discuss this source of performance degradation. 
% \end{remark}
%
% \begin{remark}{\bf No $K'>K$}
%
% \sr{say we assume no two paylodas are the same}
% \end{remark}
%
% \vspace{3cm}
%
% Next, we wish to define a code for the  A-channel and its variation above. 
% %
%Following the notation of \cite{amalladinne2018coded}, we next describe a binary linear code for the UACE as follows.
%
%Here the binary vector representation of Sec. \ref{sec:Binary representation} will be particularly useful. 
% \sr{we don't need a definition of capacity here}

% \medskip

% \begin{itemize}
% \item $L$: number of coded sub-blocks 
% \item $J$: Length of coded sub-blocks
% \item $B$: message length in bits
% \item $N$: Length of coded $B$-bit message, $N = LJ$     
% \end{itemize}

% \subsection{Objectives}
% This model can be used for stitching sections in a coded compress sensing (CCS) code. 
% % 

% For this scenario, we wish to understand the trade-off between the length of the list produced by the CCS code versus the rate allocated to the stitching code. 
% % %

% \sr{complete}
% More specifically, take a code for the unsourced MAC channel, then every unsourced $K$-user code for $B$ bits at block-length $N$  can be extended to a code of length $LB \Rsf_A$ for bits by concatenating with an outer unsourced A-channel code of rate $\Rsf_A$ with n A-channel uses.


% Ultimately, to minimize the per-user error probability, one is interested in choosing

% \begin{itemize}
%     \item the rate of the CCS code: $\Rsf_{\rm CCS}$
%     \item the length of the list of possibly transmitted codeword for the section: $l \in [L]$ $\Nsf_l$
%     \item the rate of the stitching code $\Rsf_{\rm A}$
%  \end{itemize}


\subsection{Linear codes}
\label{sec:Linear codes}
%
% Def. \ref{def:code} is rather general: in actuality, linear codes of offers a more practical class of code in terms of decoding algorithms. Let us introduce some notation for these codes here. 
% %
% The notation introduced here shall be convenient for introducing the LLC in Sec. \ref{sec:Linked-loop code}. 
%
%\subsection{Encoding}
%Assume that user/encoder $k \in [K]$ has a payload $\wv_k$ of $B$ bits to be transmitted over the UACE. 
%
%Without loss of generality, we can assume that $\wv_k$ is drawn uniformly at random over $[2]^{B}$.
%
Binary linear codes are a special case of the class of codes in Def. \ref{def:code} in which the encoding function of \eqref{eq:encoding fun} is a matrix multiplication over $GF(2)$.
%
More precisely, a binary linear code is defined as a set of $L$ %\emph{parity check  matrices} 
\emph{generator matrices}
$\{\Gv_l\}_{l \in [L]}$  which specify how the parity bits for section $l \in [L]$ are generated from the payload $\wv$. 
%
Let $\{m(l)\}_{l\in [L]}$ with $\sum_{l \in [L]} m(l) = B$ indicate the number of information bits allocated to section $l \in [L]$, and recall that $\mv = [m(0),m(1), \ldots, m(L-1)]$
%
%The size of the parity check matrices is then $\Gv_l \in [2]^{B \times(J-m(l))}$ for $l \in[L]$. 
%
Next, we partition the payload $\wv$ into $L$ vectors,
\ea{
\wv = \wv(0) . \wv(1) \ldots  \wv(L-1),
\label{eq:payload partition}
}
with $\wv(l) \in [2]^{m(l)}$ for all $l\in [L]$.
Let the parity bits in section~$l$ be denoted by $\pv(l) \in \mathbb{F}_2^{p(l)}$, where length $p(l)=J-m(l)$. 
%
% Each section $l \in [L]$, we assume that the  there are $w(l)$ information bits and $p(l)$ parity bits.
% The length of the two parts is 
% \eas{
% |w(l)|  & = m(l) \\
% | p(l)| & =  J-m(l),
% }
% that is, the $l$ section carries $m(l)$ information bits, the rest are parity bits. 
% %
%
The parity bits are obtained from the payload as
\eas{
\pv(l) &= \wv \Gov_{l}  \\
&= \sum_{l' \in [L]} \wv(l') \Gv_{l'l},
\label{eq:parity equation 2}
}{\label{eq:parity equation}}
where $\Gov_{l} \in \mathbb{F}_2^{ B \times (J-m(l))}$.
%
When considering the partitioning of the payload as in \eqref{eq:payload partition}, one naturally obtains a partitioning of the $\Gov_{l}$ in sub-matrices  as in \eqref{eq:parity equation 2} where $\Gv_{l'l} \in \mathbb{F}_2^{m_{l'} \times (J - m(l))}$. 
%are parity check matrices and the summation is over $\rb{GF}_2$.
%
%We do not explicitly indicate the dimensions of $G_{ll'}$.
%
Finally, the channel input is obtained as 
\ea{
\vv(l) = \wv(l).\pv(l).
}
The parameters found in this section are summarized in Tab.~\ref{tab:DNN parameters}.

\begin{figure}
    \centering{\include{figures/codeword}}
    \vspace{-0.75cm}
    \caption{This notional diagram depicts the formation of a linked-loop codeword.}
    \label{fig:codeword}
\end{figure}

\begin{remark}
Throughout the section, we have omitted the subscript $k$ found in \eqref{eq:input binary size N}.
This simplifies notation and it stresses the fact that the encoding is the same at all users $k \in [K]$.
\end{remark}

\begin{table}
	\footnotesize
	\centering
	\vspace{0.04in}\caption{Relevant Symbols and Parameters}
 %{This table contains key parameters encountered}
	\label{tab:DNN parameters}
	\begin{tabular}{|c|c|}
		\hline
        Notation & Parameter Description \\ \hline
		%$K_a$ & Number of active users  \\ \hline
        $B$ & Message length in bits \\ \hline
        $L$ & Number of coded sub-blocks per round \\\hline
        $J$ & Length of coded sub-blocks  \\ \hline
        $N$ & Length of coded $B$-bit message, $N=LJ$ \\ \hline
        $M$ & Number of previous sub-blocks used to generate parity bits\\ \hline
        $m(l)$ & Number of information bits in $l$-th sub-block \\ \hline
        $p(l)$ & Number of parity bits in $l$-th sub-block, $p(l) = J-m(l)$ \\ \hline
	\end{tabular}
	% \vspace{-0.5cm}
\end{table}



%
%\sr{say all users have the same encoding again}
% %
% \subsection{Motivation and Further comments}
% \label{sec:Motivation and Further comments}

% The UACE  finds its application in the URA-channel as in \cite{amalladinne2018coded} in which AMP decoding returns a list of estimated active payload in each section $[L]$. 
% %
% In its original analysis, the authors of \cite{amalladinne2020coded} assume that this list contains all active payloads plus some hallucinated payloads. 
% %
% The UACE allows one tackle the scenario in which the AMP decoder outputs a list that misses some of the active payloads.
% %
% The UACE, does not capture the full complexity of a stitching code for CCS as it does not consider both \emph{insertions} and deletions. 
% %
% % Such a model is expressed as a variation of \eqref{eq:channel error}
% % \ea{
% % Y = \bigcup_{k \in [K]}  \delta_{E_{k}} (x_{k})
% % %\lb X_{lk} E_{lk} + (1-E_{lk}) \emptyset \rb,
% % \label{eq:channel error}
% % }
% The unsourced A-channel with insertions and deletions is left for future research. 
% %
% Finally, another interesting variation is the one in which  the erasures $E_{l,k}$  are correlated in $k$. 
% %
% This model would be relevant in the case of an unsourced MAC channel with fading.

% % \sr{does this correspond to the group testing when one of the test is missing? that'll actually be pretty cool}
% % \subsection{Further comments}

% % \begin{itemize}[leftmargin=*]
% %     \item  {\bf  Unsourced A-channel with errors, insertion, and deletion}
% %     \item  {\bf type I and type II errors}
% %     \item {\bf correlated erasures coming from URA with fading}
% %     \item ? 
% % \end{itemize}





==> conclusion.tex <==

\section{Conclusion}
This paper presents a novel coding scheme designed for UACE called linked-loop code (LLC). The LLC is managed to identify all payloads suffer no erasure, also to recover payloads suffer one erasure from the UACE. The latter greatly decreases PDP, while keeping PHP to be empirically low comparing with some other methods in the recent literature. 




==> intro.tex <==
\begin{abstract}
    
The A-channel is a noiseless multiple access channel in which users simultaneously transmit $Q$-ary symbols and the receiver observes the set of transmitted symbols, but not their multiplicities. 
%
An A-channel is said to be unsourced if, additionally, users’ transmissions are encoded across time using a common codebook and decoding of the transmitted messages is done without regard to the identities of the active users \cite{lancho2022finite}.
%
An interesting variant of the unsourced A-channel is the unsourced A-channel with erasures (UACE), in which transmitted symbols are erased with a given independent and identically distributed probability. 
%
In this paper, we focus on designing a code that enables a list of transmitted codewords to be recovered despite the erasures of some of the transmitted symbols. 
%
To this end, we propose the linked-loop code (LLC), which uses parity bits to link each symbol to the previous $M$ symbols in a tail-biting manner, i.e., the first symbols of the transmission are linked to the last ones. 
The decoding process occurs in two phases: the first phase decodes the codewords that do not suffer from any erasures, and the second phase attempts to recover the erased symbols using the available parities. 
We compare the performance of the LLC over the UACE with other codes in the literature and argue for the effectiveness of the construction. 
Our motivation for studying the UACE comes from its relevance in machine-type communication and coded compressed sensing.

{\ste update and complete}
\end{abstract}

\begin{IEEEkeywords}
A-channel; A+ channel; Unsourced random access; code design. 
\end{IEEEkeywords}

\section{Introduction}

%This paper studies  ``the Gamblers' Anonymous Betting Problem'', which has wide connections to communication, computer science, and optimization. The problem can be best illustrated through an example: 

The problem is better stated through an example. Assume that a group of gamblers wish to anonymously submit their bets to a bookmaker for horse races occurring throughout the day. Each bet consists on the number of the winning horse. The bets  collected by the bookmaker anonymously throughout the day and payouts are handed out at the end of the day. In order to avoid cheating, the bookmaker decides ahead of time some rules that the gamblers have to follow in their betting, so that all the bets of a given gambler can be collected and paid out anonymously. 
%
For example, it declares that in the third race, each gambler has to bet on a horse number which is the sum of the first two horses the gambler placed bets on. If all gamblers follow the rules, the bookmaker can then payout a gambler by asking only what was the bet on the third horse. 
%
The question that we want to ask is as follows: Given a certain number of horses, gamblers, and races in a day, how many bets can a gambler place freely? The problem as stated shows clear connections to a number of combinatorial problems, from 


{\ste Jamison will rewrite as a more communication me}

% Imagine a group of gamblers who want to anonymously submit their bets for a day of horse races to a bookmaker. Each gambler places bets on the winning horse numbers. To ensure anonymity, the bookmaker sets rules for the bets, such as requiring gamblers to bet on a horse number that is the sum of the first two horses they placed bets on. The goal is to determine how many bets a gambler can freely place given the number of horses, gamblers, and races in a day. This problem encompasses combinatorial aspects and has connections to communication, retrieval, and optimization. Despite some specific scenarios being addressed in the literature, the general solution to this problem remains open. This project aims to contribute significantly to advancing our understanding and finding solutions for this intriguing problem.

% Keywords: coding techniques, Gamblers' Anonymous Betting Problem, communication, computer science, optimization, anonymity, horse races, combinatorial problems, sabbatical research, funding proposal.



In this case, the group chat can be seen as an analogy to the A-channel. Each friend represents a user, and the messages they send correspond to the symbols being transmitted. The chat platform displaying the messages in a jumbled order without identifying the senders or message repetitions is similar to the receiver in the A-channel model, which observes the transmitted symbols but lacks information about their multiplicities or the identities of the senders.
This example highlights the relevance of the unsourced A-channel model in scenarios where multiple users transmit information simultaneously, but the receiver can only observe the symbols without knowing their multiplicities or the identities of the users. This model is applicable to various real-world situations, including machine-type communication, IoT devices, and other scenarios where efficient handling of simultaneous transmissions is required.


{\ste chatGPT output}


\vspace{2cm}
from the original paper


possible.
Two specific channel models are considered. They will be referred to as the T-user M-frequency multiple-access
channel with (or without) intensity knowledge. For ease of future reference, the channel without intensity knowledge will be referred to as the A channel while the channel with
intensity knowledge will be referred to as the B channel. 

{\ste right name is A channel and B channel}


\vspace{2cm}

    The A-channel with erasures is defined by the input/output relationship 
    \ea{
    \textstyle Y = \bigcup_{k \in [K]}  \delta_{E_{k}} (x_{k}),
    %\lb X_{lk} E_{lk} + (1-E_{lk}) \emptyset \rb,
    \label{eq:channel error}
    }
    where the $k$th users's symbol $x_{k} \in \Qcal, |\Qcal|=Q$,
    %[Q] = \{1, \ldots, Q\}$, 
    %
    the erasure indicator $E_{k} \stackrel{\text{iid}}{\sim} \Bcal(p_e)$, and the erasure function is defined as 
    \ea{
    \delta_{E}(x) \coloneqq \lcb \p{
    x  &  E = 0  \\
    \emptyset & E = 1.
    }\rnone
    }
    Above, $\Bcal(p)$ indicates the Bernoulli distribution with parameter $p_e \in [0,1]$.
    %\wz{we need to say what is $l$ here.}
    % SR2WZ: dropped
    % SR2WZ: I think you misunderstood the set comment in the last meeting. see how i did it.
    %
    % \sr{change this to an input to a given cardinality}
    %
    %\sr{change the notation for}
In the A-channel with erasures of \eqref{eq:channel error},
%is the multiple-access channel (MAC) where each of $K$ users transmits a symbol from a set $\Xcal$ with cardinality $Q$, and 
each symbol is received by the receiver with probability $1-p_e$ and erased with probability $p_e$. 
%
%In other words, the A-channel with erasures of \eqref{eq:channel error} is the channel  model in which each user $k \in [K]$ transmits a symbol from the alphabet $\Xcal$ where $\Xcal$ is a set of cardinality $Q$. 
    %
%This symbol is correctly communicated at the receiver with probability $1-p_e$ and is otherwise erased. 
%
The unsourced A-channel with erasures (UACE) is similar to the model described in \eqref{eq:channel error}; however, the receiver is only interested in identifying the transmitted codewords, rather than the traditional source-message pairs. 
%This is particularly useful in scenarios with short-packet random access wireless communication, as it eliminates the need for user enrolment.
% %
% In this article, we introduce the UACE paradigm, and we propose a coding scheme for the challenge which we term linked-loop code (LLC). 
% % The LLC uses parity bits to link coded symbols in a tail-biting manner, allowing for decoding of codewords that were not erased in the first phase of decoding, followed by recovery of erased symbols in the second phase.
% The LLC uses parity bits to link coded symbols in a tail-biting manner, thus allowing for codewords to be recovered even when some of their symbols have been erased.
% We evaluate the performance of the LLC and compare it to that of other coding schemes available in the literature.
    
%     Motivated by the short-packet random access wireless scenario, we consider the scenario in which the receiver is interested only in knowing which codewords have been transmitted but not by which user. 
%     %
%     This paradigm is useful as it removes the need for user enrolment, which is too taxing when the payload is short.
%     %
%     We refer to this transmission setting as the unsourced A-channel with erasures (UACE).
%     %
%     % \vspace{2cm}
%     %
%     %
%     % Motivated by the short-packet random access wireless scenario for massive machine-type communications, we consider the scenario in which the transmitters use a common codebook of length $N$ 
%     % % \wz{We seldomly use "N"}
%     % while the receiver is interested only in knowing which codewords have been transmitted, but not by which user. 
%     % %
%     % We refer to this transmission setting as the unsourced A-channel with erasures (UACE).
%     % %
    
%     In this paper, we (i) introduce the UACE and (ii) design the first coding scheme for recovering erased symbols which we refer to as the linked-loop code (LLC). (iii) The performance of the LLC is evaluated and compared to other schemes available in the literature. 
%     %
%     %
%     % $K$ users in transmit symbols from a $Q$-ary input alphabet $[Q]$ over a MAC channel with input/output relationship at time $t \in [T]$ is defined as 
%     % \ea{
%     % Y_t = \bigcup_{k \in [K]} X_{lk},
%     % \label{eq:channel perfect}
%     % }
%     % where $x_{lk} \in [Q]$
%     % To indicate the set of outputs $\{Y_t\}_{t \in [T]}$ we use the vector notation $\Yv$.
%     %
    
    
% \subsection{Literature Review}
% \label{sec:Literature Review}

\noindent
\textbf{Literature Review:}

The A-channel is described in \cite{chang1981t}, where it models a multiple-access channel that employs frequency division for transmission without the availability of signal intensity. 
The authors of \cite{chang1981t} determine the mutual information of the A-channel under uniform inputs. 
The limit of the mutual information of the A-channel when $K$ and $Q$ tend to infinity, with the ratio $\lambda = K/Q$ kept fixed, is studied in \cite{bassalygo2000calculation}.
%
Recent interest in the A-channel is due to the emergence of short-packet machine-type communication and IoT devices.
In particular, the idea of unsourced random access (URA) is introduced in \cite{polyanskiy2017perspective} as an alternative to the customary identify-then-transmit procedure. 
%
% In the URA-channel, the unsourced A-channel is used as part of the code design as it allows the transmission block-length to be partitioned into multiple sections.
A common strategy in URA is to use concatenated coding techniques; when this strategy is adopted, in certain settings, the unsourced A-channel can serve as an abstraction for the channel between the outer encoders and the outer decoder. 
%
For example, in \cite{amalladinne2020coded}, a linear inner code is used to further encode outer-encoded messages, where the outer code allows for recovery over the unsourced A-channel. 
%
% The parity bits are obtained from a code that allows recovery over the unsourced A-channel. 
%
During inner decoding, each section is decoded independently, and a list of outer codeword symbols is produced for each section. 
The parity bits from the outer code designed for the unsourced A-channel are then used to link the outer codeword symbols corresponding to the same user across all the transmission sections.
%
The ensuing unsourced A-channel code is termed the tree code.
The original tree code has been enhanced in \cite{amalladinne2020coded,amalladinne2021unsourced}.
% 
More recently, following the renewed interest in these applications of the A-channel, Lancho et al.~\cite{lancho2022finite} offered finite-blocklength achievability bounds for the unsourced A-channel.
%
% At decoding, each section is decoded independently and a list of possible transmitted messages is produced for each section. 
% %
% The parity bits from the A-channel are then used to link the information bits from the same user across sections.
%
% This transmission scheme uses a random inner code of size $Q$ concatenated with an outer $Q$-ary A-channel
% code. 
%
%This is attained by using a linear code to encode information and parity bits over each section, and a code that allows recovery over the A-channel to obtain the parity bits. At decoding, each section is decoded independently, and a list of possible transmitted messages is produced for each section. The parity bits from the A-channel are then used to link the information bits from the same user across sections.
%
%The section also highlights the coded compressed sensing (CCS) approach introduced in \cite{amalladinne2018coded}, which employs a random inner code of size $Q$ concatenated with an outer $Q$-ary A-channel code for URA over an AWGN channel. 
%and is constructed to be flexible for use in different channel models. 
% Several follow-up works on URA have further elaborated on this approach 
%
%The section concludes by discussing recent work on finite-blocklength achievability bounds for the unsourced A-channel in \cite{lancho2022finite}.
%
% %
% The A-channel was originally introduced in \cite{chang1981t} to model a multiple-access channel model where frequency division is used for transmission but where the intensity of the signal over each frequency is not available. 
% %
% The authors of \cite{chang1981t} determine the mutual information of the A-channel under uniform inputs.
% %
% Its limit when $K$ and $Q$ tend to infinity but its ratio $\lambda = K/Q$ is fixed was studied in 
% %\wz{I think we'd double check these notations, or use notations related in our work} 
% % SR? we have K and Q here as well. 
% \cite{bassalygo2000calculation}.
% The mutual information with uniform inputs in the sparse limit of $K,Q \goes \infty$  with fixed ratio $(\log K)/Q$
% was computed in \cite{fengler2021sparcs} and it was shown that in this limit the
% mutual information grows proportional to $\log Q$.
% %
% More recently, the A-channel has found renewed interest in the literature due to the emergence of short-packet machine-type communication and the IoT paradigm. 
% %
% Consider the scenario in which a large number of devices wishes  to communicate a small payload to a central server.
% %
% When the payload is so short, the customary identify-then-transmit procedure  in which each user uses a control channel to obtain a network resource becomes inefficient.
% %
% %
% On the other hand, freely accessing the medium causes  collisions among the transmissions that can only be resolved through a feedback signal, which also requires too much coordination. 
% %
% An alternative paradigm to these two approaches is that of the unsourced random access (URA) channel \cite{polyanskiy2017perspective}. 
% %
% In the URA-channel, users transmit using the same codebook so that  the receiver can only recover a list of transmitted codewords up to permutation. 
% %
% The A-channel played an important role for codes design in URA as it allows the transmission block-length to be partitioned in multiple sections. 
% %
% This is attained as follows \cite{amalladinne2020coded}.
% %
% Over each section, a linear code is used to encode information and parity bits. 
% %
% The parity bits are obtained from a code that allows recovery over the A-channel. 
% %
% At decoding, each section is decoded independently and a list of possible transmitted messages is produced for each section. 
% %
% The parity bits from the A-channel are then used to link the information bits from the same user across sections.
% %
% % This transmission scheme uses a random inner code of size $Q$ concatenated with an outer $Q$-ary A-channel
% % code. 
% %
% In \cite{amalladinne2018coded}, a coding scheme for AWGN URA termed coded
% compressed sensing (CCS) was introduced. 
% % %
% % This transmission scheme uses a random inner code of size $Q$ concatenated with an outer $Q$-ary A-channel
% % code. 
% % %
% % In a CCS code, generally speaking,  compressed sensing algorithms are used to determine the list of codewords present in the channel output. 
% % %
% % The complexity of these compressed sense algorithms is rather large, so that long block lengths are not feasible from a numerical perspective. 
% %
% The A-channel code constructed for this purpose was termed tree code. The flexibility of this code construction
% allowed it to be extended to different channel models. Several follow-up works on URA have further elaborated on this approach \cite{amalladinne2020coded,amalladinne2021unsourced}
% %
% More recently, following the renewed interest in these applications of the A-channel, the authors of \cite{lancho2022finite} present finite-blocklength achievability bounds for the unsourced A-channel.

% %\sr{put some of our papers here}
% %
% %
% % \vspace{5cm}
% %
% % packets. Since its
% % inception, this problem has been commonly referred in the
% % literature as unsourced random access (URA). Several papers
% % establishing fundamental limits for different relevant multiple access
% % channel models and setups appeared since then (see,
% % e.g., [6]–[9]), and
% %
% % The A-channel finds interesting applications in noiseless
% % non-adaptive group testing.
% %
%
%
%\subsection{Contribution}

\noindent
\textbf{Contributions:}
%
%In this paper, we provide the following contributions:
The major contributions of this article can be summarized as follows.
\begin{itemize}[nolistsep,leftmargin=*]
    \item  {\bf Sec.~\ref{sec:Channel Model} :} We introduce the UACE model, we define the information transmission problem for this model, and we identify relevant performance metrics. 
    %In particular, the error probability analysis is comprised of two terms: the probability that a message declared as transmitted is not transmitted 
    %
    %performance is measure in term
    %provide motivation for this model.
    %
    
    \item {\bf Sec.~\ref{sec:Linked-loop code} :} We propose the linked-loop code
(LLC) as the first code specifically designed for the UACE. Encoding and decoding procedures are described. The code parameters are also discussed. 

\item {\bf Sec.~\ref{sec:Related Results} :} We review codes in the literature that are compatible with the UACE setting, although not specifically designed for this channel: (i) the tree code of \cite{amalladinne2020coded}, and the (ii) outer LDPC code (triadic design) of \cite{amalladinne2021unsourced}. 
%
%These two codes are used for numerical comparison of performance in Sec. \ref{sec:Simulation Results}.

\item {\bf Sec. \ref{sec:Simulation Results} : } Numerical simulations offer insight into the performance of the LLC in Sec.~\ref{sec:Linked-loop code}, and we provide a performance comparison with other systems in Sec.~\ref{sec:Related Results}.
\end{itemize}
%Finally, Sec. \ref{sec:Conclusion} concludes the paper. 
%SR: no conclusion

%\textit
{
\medskip
\noindent
{\bf Notation:} 
%
In the following, 
%lowercase boldface letters (eg. $\zv$) are used for row vectors and uppercase boldface letters (e.g., $\Mv$) designate matrices. 
%
%Sets are indicated with calligraphic letters. 
%
%The all-zero vector of dimension $d$ is indicated as $\zerov_d$.
%
%We also 
we adopt the short-hand notation 
%$[m:n] \triangleq \{m, \ldots, n-1\}$
%and
$[N] \triangleq (0, \ldots, N-1)$. 
%
%The $p$-norm of the vector $\xv$ is indicated as $\| \xv\|_p$.
%
%Random variables are indicated with uppercase letters, e.i. $N$. 
%With $|\Scal|$ we indicated the cardinally of the set $\Scal$.
%
%  \vspace{1cm}
% {\color{blue}SR: complete here.}
% \vspace{1cm}
%
% %
% Subscripts are used for node indices and parentheses depict iteration index (eg. $\zv_i(k)$ denotes the state of node $i$ at iteration $k$).
% %
% $\overline{\Paren{\cdot}}$ denotes the average of corresponding quantities across different nodes and $\widehat{\Paren{\cdot}}$ is used for iteration-averaged quantities. 
% %
% The noisy version of a variable is indicated with a tilde, i.e. $\widetilde{\av}$ is the version of $\av$ after being corrupted by noise.
% %
% For any arbitrary norm $\norm{\cdot}$, its dual norm is defined as $\norm{\cdot}_* = \sup_{\xv: \norm{\xv} \leq 1} \inprod{\cdot, \xv}$, where $\inprod{\cdot,\cdot}$ denotes the inner product.
% %
% We primarily consider Euclidean norm  $\norm{\cdot}_2$ in this work, which is its own dual.
% \iffalse
% {\color{red} norm and $\langle$, $\rangle$ need to be connected}
% \fi
% %
% Given a sub-differentiable function $f$, its sub-differential at $\xv$ is denoted by $\partial f(\xv)$.
% %
Calligraphic scripts are used to denote sets (e.g., $\Acal$), and $|\cdot|$ is used to denote the cardinality of a set.
%
$GF(2)$ indicates the Galois field of order 2.  
%
Given two row vectors $\vv$ and $\wv$, we denote their concatenation as $\vv.\wv$.
% \sr{double check what's needed}}
% \sr{say we use vector and set notation interchangeably when creates no confusion3}
% \sr{add notatiton concatenation of string $.$}
%
Random variables are indicated with uppercase letters (e.g., $N$). 
% With $|\Scal|$ we indicated the cardinally of the set $\Scal$.
%
With a certain abuse of notation, we sometimes interchange the notation for (random) vectors and sets when this is clear from the context. 
%
%For instance in \eqref{eq:channel error}  we indicate the channel output as a random vector, rather than a set. This is done mostly to simplify the notation. 
%represents vectors as sets and viceversa. 

%\vspace{1cm}
\medskip
\noindent
The code for the numerical evaluations of this paper is provided online at \url{https://github.com/williamzheng0711/URAC23}.
%\sr{2WZ: complete}. 


==> proposed_approach.tex <==

\section{Linked-loop code (LLC)}
\label{sec:Linked-loop code}


%
We now discuss the task of correctly identifying active payloads before introducing the LLC approach. 
For simplicity, let us consider the regime in which each user experiences no erasures.
%or only one erasure across the $L$ sections.
%
Also, we will assume no payload collision occurs, as the probability of this event is orders of magnitude smaller that the target PDP and PHP.


% The decoder considers all the list entries in section $0$, which is referred to as $\Lcal_0$. 
The decoder begins by selecting a single entry of $\yv(0)$, and sets this entry as the root of a tree. 
Then, the decoder checks all entries in $\yv(1)$ and identifies those entries that are parity consistent with the root entry. 
For each such entry, the decoder creates a path from section $0$ to section~$1$. 
% Then, the decoder extracts the information bits from  each entry in $\Lcal_0$ and checks which entries in the list of section $1$, denoted $\Lcal_1$ are parity consistent with the information bits of entries in section $\Lcal_0$. 
%
% The decoder then adds these entries to a list, which is referred to as $\Lcal_1$.
%
% Third, at the next iteration, the decoder uses the information bits in $\Lcal_0$ and entry in $\Lcal_1$ to extract a list of parity-consistent entries in section $2$, which is referred to as $\Lcal_2$. Finally, the decoder repeats this procedure until the last section $L-1$.
Proceeding, the decoder checks all entries in $\yv(2)$ and identifies those entries that are parity consistent with the previously identified partial paths through $\yv(0)$ and $\yv(1)$. 
Retaining only parity-consistent paths, the decoder proceeds until all sections have been considered. 
In the tail-biting scenario, the first sections may need to be re-considered to ensure that they are parity-consistent with the last sections. 
The hope is that, by the end, a single parity-consistent path remaining, which corresponds to a transmitted codeword. 
As in \cite{amalladinne2020coded}, we refer to this operation as \emph{stitching} and illustrate the algorithm in Fig.~\ref{fig:stitching}. 

%
% Following \cite{amalladinne2020coded}, let us refer to this operation of "linking" parity-consistent list entries across multiple sections as \emph{stitching}. Also, call the set of stitched elements in each section a \emph{path}. A path starts with an entry (referred to as "root") in the list of section $0$, then stitches some parity-consistent element from the list of section $1$, and so forth. A graphical representation of this process is provided in Fig. \ref{fig:stitching}.


% \vspace{5cm}

% The decoder can decode an active payload by following these steps. First, the decoder selects one of the list entries in section $0$, which is referred to as $\Lcal_0$. Second, the decoder extracts the information bits from this section and checks which entries in the list of section $1$ are parity consistent with the information bits in section $0$. Generally speaking, there can be a number of parity-consistent entries, so the decoder adds these entries to a list, which is referred to as $\Lcal_1$. Third, at the next iteration, the decoder uses the information bits in $\Lcal_0$ and every entry in $\Lcal_1$ to extract a list of parity-consistent entries in section $2$, which is referred to as $\Lcal_2$. Finally, the decoder repeats this procedure until the last section $L-1$.

% Following \cite{amalladinne2020coded}, let us refer to this operation of "linking" parity-consistent list entries across multiple sections as \emph{stitching}. Also, call the set of stitched elements in each section a \emph{path}. A path starts with an entry (referred to as "root") in the list of section $0$, then stitches some parity-consistent element from the list of section $1$, and so forth. A graphical representation of this process is provided in Fig. \ref{fig:stitching}.

% From the discussion above, it is clear that a computationally efficient linear code for the UACE is one in which the information bits used to generate the parity bits only cover a small number of sections so that the number of stitched elements across lists $\Lcal_l$ does not grow exponentially as the stitching process continues.

% In practice, it is more efficient to link all paths starting from the root entries and proceed sequentially, section after section. This is because parity-consistency for all paths can be formulated as a single matrix multiplication. We refer to this decoding phase as \emph{phase 1} in the following.

Next, let us discuss a decoding approach when only one erasure is encountered. 
When an erasure occurs for a certain user, the decoder is not able to insert the correct element in one of the lists, let's say $\yv_l$. 
Consequently, the number of surviving paths becomes zero for some section $l'$ with $l \leq l' \leq L$. 
This means that, after all initial paths have been linked, some of the elements of the root do not have a complete path of length $L$. For these remaining codewords, a \emph{phase 2} of decoding is needed in which all non-terminating paths are considered.
% In phase $2$, we consider only non-terminating paths in phase $1$. 
For these paths, we introduce a special symbol, $\na$, that enables each path to have a one-section loss tolerance. 
After all other sections not in outage have been stitched to some path, we calculate the lost section's information bits by reverse-engineering \eqref{eq:parity equation}.

%When introducing binary linear codes in Sec.  \ref{sec:Linear codes} we only discussed the encoding operation but not the decoding one. 
%
%and consider the inherent difficulty in correctly identifying the payloads so as to minimize the PUPE as in Def. \ref{def:pupe}. 
% %
% Let us briefly discuss the inherent difficulty in correctly identifying active payloads so as to minimize PDP and PHP before introducing the proposed approach. 
% %
% For simplicity, let us consider the regime in which
% %, with high probability, 
% each user experiences either no erasures or only one erasure across the $L$ sections. 
% %
% %If no erasure is experienced through the transmission by any of the $L$ sections, the decoder can proceed as follows:
% The decoder can decode an active payload as follows.
% %
% First (i) pick one of the list entries in section $0$, call it $\Lcal_0$ 
% (ii) extract the information bits from this section and check which entries in the list of  section $1$ are parity consistent with  the information bits in section $0$. Generally speaking, there can be a number of parity-consistent entries, so add these entries in a list, let's call this list $\Lcal_1$. (iii) at the next iteration, use the information bits in $\Lcal_0$ and every entry in $\Lcal_1$ to extract a list of parity-consistent entires in section $2$, call this $\Lcal_2$. (iv) Repeat (iii) until the last section $L-1$. 
% %

% Following \cite{amalladinne2020coded}, let us refer to this operation of  ``linking'' parity-consistent list entries across multiple sections as \emph{stitching}. Also call the set of stitched elements in each section a \emph{path}. A path starts with an entry (referred as "root") in the list of section $0$ then stitch some parity consistent element from the list of section $1$ and so forth. A graphical representation of this process is provided in Fig. \ref{fig:stitching}.
% %
% % More specifically, one  user can select one element in any of the channel outputs and extract the information bits from this given section. 
% % %
% % The decoder can then check for the elements in the list of the following section which are parity consistent with the information bits using \eqref{eq:parity equation}. 
% % %
% % Possibly multiple elements in this list satisfy the parity consistency: when checking for the following section, all these possible combinations have to be checked for parity consistency.
% % %
% % By repeating this procedure, the decoder finally obtains $L$ parity consistent elements and declares the corresponding payload as active. 
% %
\begin{figure}
    \centering{\include{figures/stitching}}
    \vspace{-0.75cm}
    \caption{The diagram illustrates the stitching of elements across sections.
    When successful, this process returns candidate codewords.}
    \vspace{-0.25cm}
    \label{fig:stitching}
\end{figure}
% %
% From the discussion above, it is clear that a computationally efficient linear code for the UACE is one in which the information bits used to generate the parity bits only cover a small number of sections so that the number of stitched elements across lists $\Lcal_l$ does not grow exponentially as the stitching process continues. 


% In practice, it is more efficient to link all paths starting from the root entries and proceed sequentially, section after section. This is because parity-consistency for all paths can be formulated as a single matrix multiplication. 
% %
% We refer to this decoding phase as \emph{phase 1} in the following. 

% Next, let us discuss a decoding approach when only one erasure is encountered. 
% %
% % First note that when a payload is identified as active, then the path of this payload can be removed form the channel output $\yv$. 
% % %
% % This simplifies the task of identifying the remaining active payloads. 
% % %
% When an erasure occurs for some certain user
% % a certain user $k$
% , the decoder is not able to insert the correct element in one of the lists, let's say $\Lcal_l$.
% %
% Consequently, the number of surviving paths becomes zero for some section $l'$ with $l \leq l' \leq L$. 
% %
% This means that after all initial paths have been linked, some of the elements of the root do not have a complete path of length $L$.
% %

% For these remaining codewords, a \emph{phase 2} of decoding is needed. 
% %
% In phase $2$, we consider only  non-terminating paths in phase $1$. For these paths, we introduce a special symbol, $\na$, 
% that enables each path to have a one-section loss tolerance. After all other present sections have been stitched to some path, we calculate the lost section's information bits by reverse-engineering \eqref{eq:parity equation}.
% % when a parity consistency could not be determined for the path of index $k$ in section $l$.  
% %
% % Note that the location of the erasures is known since (ignoring collisions) $|\yv|<K$ when an erasure occurs. 
% %
% % When, in the following section, parity consistency encounters an $\na$ symbol a new path is generated. 

% % \sr{william help}



% %upon encountering the section containing the erased symbol, two event can occur (i) the decoder finds a parity consistent symbol actually belonging to another user, or (ii) the decoder cannot find a parity consistent element. 
% %
% %
% % %
% % If (i) occurs, than let us assume for simplicity that the decoding process fails. \footnote{This is just a simplification \sr{complete}}
% % %
% % If (ii) occurs, the decoder is then aware of that a symbol has been erased  and proceeds in stitching the current path with all the possible information bits that are parity consistent with the current path across the decoded bits and that are not present in the current list. 
% % %
% % This process greatly increases the complexity of decoding process as it creatly increases the number of paths to be considered. 
% % %
% % To prevent this, and assuming that no collision among payloads has occurred,  the decoder can start the decoding process from the shortest list of symbols $Y_l$.
% % %which is further away from the next list of length less than $K$.
% %
% %\medskip
% %
% Having discussed the properties of a good  approach above, we shall now detail the LLC construction, encoding, and decoding. 


%\subsection{Construction}

\subsection{Encoding}
The LLC is a binary linear code for the UACE defined by: (i) a memory depth $M$,  and (ii)  a set of $M$ parity matrices $\{\Gv_r 
% \in \mathbb{F}_2^{m \times (J-m)}
\}_{r = 1}^{M}$.
%
The LLC has a fixed number of information and parity bits in each section, i.e.,
%That is, $\forall l\in [L], 
$m(l)=m$ for some $m>0$.
%
Additionally, the $J-m$ parity bits depend on the information bits of the $M$ previous sections, in a circular manner, that is 
\eas{
\pv (l) & = \textstyle  \sum_{l' \in [L]} \wv(l')\Gv_{l'l} \\
% & = \sum_{0 < l-l' \, {\rm mod} \, L \leq M } \wv(l') \Gv_{l'l} \nonumber \\
& = \textstyle \sum_{r =1}^{M} \wv( l-r \, {\rm mod} \, L) \Gv_{r},
\label{eq:parity equation 3}
}
where in \eqref{eq:parity equation 3} we have set $\Gv_{l'l}=\Gv_{r}$ for $r = l-l' \, {\rm mod} \, L$ and $1\leq r\leq M$.

% In each section, the remaining $J-m$ parity bits are depend on a fixed $M \in \{1,2, \ldots, L-1\}$ previous section in a ring manner, that is the parities in section $l$ depend on the sections  $l' \in \mathcal{D}^L_M(l) \coloneqq \{l-M' \mod{L} | 1\leq M' \leq M, M' \in \mathbb{N}^+  \}$. 
% From now on, we may use $\mathcal{D}(l)$ as a shorthand of $\mathcal{D}^L_M(l)$.

% The epression in \eqref{eq:parity equation} therefore simplifies to 
% \ea{
% \pv(l) & \equiv \sum_{\substack{l' \in \mathcal{D}^L_M(l) }} \wv(l') \Gv_{l',l}.
% \label{eq:parity equation 2}
% }{\label{eq:parity equation LLC}}
% where $\Gv_{a,b}$ denotes an $m \times (J-m)$ binary matrix.

For example, if $L=16$ and $M=2$, the first three lists of parity bits are obtained as:
\eas{
\pv(0) & =  \wv(14)\Gv_{2} + \wv(15)\Gv_{1} \\
\pv(1) & =  \wv(15)\Gv_{2} + \wv(0)\Gv_{1} \\
\pv(2) & =  \wv(0)\Gv_{2} + \wv(1)\Gv_{1}.
%\\
%\pv(3) & =  \wv(1)\Gv_{2} + \wv(2)\Gv_{1}.
}
%
%\sr{WZ:complete}.
% parities in section 3 depends on information bits in section $1$ and section 2, more precisely, 
% \ea{
% \pv(3) & = \sum_{\substack{l' \in \mathcal{D}(3) }} \wv(l') \Gv_{l',3}=\sum_{\substack{l' \in \{1,2\} }} \wv(l') \Gv_{l',3}.
% }{}
% and parities in section $1$ is determined via 
% \ea{
% \pv(1) & = \sum_{\substack{l' \in \mathcal{D}(1) }} \wv(l') \Gv_{l',1}=\sum_{\substack{l' \in \{0,15\} }} \wv(l') \Gv_{l',1}.
% }{}

% (\sr{checx this, i'b just guessing atm...})


\subsection{Decoding}

% Following the discussion above, let us consider a two phase decoding algorithm: 
% \begin{itemize}[leftmargin=*]
%     \item \emph{phase 1:} the receiver identifies and decode the active payloads which suffer no erasures in any of the $L$ sections. 
%     \item \emph{phase 2:} the receiver attempts to identify and recover the active payloads which suffer erasure on only one section.
% \end{itemize}

% For simplicity of exposition,  we consider the case in which the receiver randomly selects the elements to place in $\whv$ for all the payloads that are not recovered after phase 2. 

% \sr{2WZ: complete here. add a nice picture}
%
%
% \subsubsection{Phase 1}
% \label{sec:Phase 1}

% In phase 1, we do the following for each entry $x_0 \in \bold{y}_0$ in list of section 0. Note that only if a path have stitched section $0, \ldots ,M-1$, we can for the first time calculate some parity, that is $\bold{p}(M)$. Hence we will keep all possible path up to section $M-1$ in our $$\Lcal_{M-1}^1(x_0)=\{[x_0, \ldots, x_{M-1}] |x_l \in \bold{y}_l, \forall 1\leq l \leq M-1 \}.$$
% %
% We update to $\Lcal_M^{1}(x_0)$ by stitching each path in $\Lcal_{M-1}^1(x_0)$ with parity consistent entries in section $M$ and discarding paths that do not admit a stitching. Repeat this process until we get $\Lcal_{L-1}^1(x_0)$. 
% %
% For each path $\in \Lcal_{L-1}^1(x_0)$, we check the parity consistency of section $[M]$, since we did not check them when we stitched them on, to obtain $\Lcal^{1}(x_0)$ by dropping inconsistent paths. 
% %
% Where inconsistent path refers to a path having some section known to be inconsistent according to \eqref{eq:parity equation 2}. All information bits of the elements in $\Lcal^1\coloneqq \bigcup_{x_0 \in \yv_0} \Lcal^1(x_0)$ will be extracted as decoded messages, constituting a set $\bold{\widehat{W}}_1$.

% \sr{still have to check}

% \subsubsection{Phase 2}

% For phase 2, we only choose those $x_{0}^\times \in \bold{y}_0$ such that $x_{0}^\times$ does not give rise to any decoded message in phase 1 to be roots. 
% % Because two users' messages sharing the same section 0 is by nature not probable, while doing this hugely reduces the complexity. 
% After we've fixed a root $x_{0}^\times$, we then proceed almost the same as in phase 1. 
% %
% The only difference is that we have a one-section erasure tolerance. That is for all $l\in[L-2]$, when we update our $\Lcal_l^2(x_{0}^\times)$ to $\Lcal_{l+1}^2(x_{0}^\times)$, for any path $\in \Lcal_l^2(x_{0}^\times)$, if that path has not contain an $\na$, we make a copy of that path and stitch an $\na$ onto its section $l+1$, no matter this path has a parity consistent entry in the list of section $l+1$ or not. This new path with $\na$ will also be an element of $\Lcal_{l+1}^2(x_{0}^\times)$. Keep doing this until we eventually end up with $\Lcal_{L-1}^2(x_{0}^\times)$. 
% % 
% Then we prune $\Lcal_{L-1}^2(x_{0}^\times)$ to $\Lcal^2(x_{0}^\times)$ by discarding all inconsistent paths of $\Lcal_{L-1}^2(x_{0}^\times)$ and calculate the lost section's information bits. Similar to phase 1, all elements of 
% $$\Lcal^2\coloneqq \bigcup_{x_{0}^\times \in \yv_0} \Lcal^2(x_{0}^\times)$$ 
% will be extracted their information bits and those resultant messages forms a set $\widehat{\Wv}_2$. Finally,
% $$\widehat{\Wv} \coloneqq \widehat{\Wv}_1 \cup \widehat{\Wv}_2$$ is our set of decoded messages.

% Now let us see in detail how a payload suffer only one erasure is recovered. Suppose a codeword $\vv=\vv(0). \ldots .\vv(L-1)$ has its section $l \in [L]$ erased by UACE, while all other sections are present. 
% % 
% In this case, we must have an element 
% $$[\vv(0),\vv(1),\ldots,\underbrace{\na}_{\text{section $l$}},\ldots,\vv(L-1)] \in \Lcal^2(\vv(0)) \subset \Lcal^2$$
% after phase 2.
% If we can uniquely determine $\bold{w}(l)$, the information portion of $\vv(l)$, then we are done. The following $M$ equations deduced by reverse-engineering \eqref{eq:parity equation 2} enable us to do so. That is
% $\forall \iota : 0< (\iota - l) \mod{L} \leq M
% % \in \{l+M' {\rm mod} L : M' \in [1,M], M' \in \mathbb{N}^+\}
% $,
% \begin{equation}
%     \bold{w}(l)\bold{G}_{l,\iota}=\bold{p}(\iota )-\sum_{\substack{l' \neq l \\ l':0 < (\iota-l') {\rm mod} L \leq M} }\bold{w}(l')\bold{G}_{(\iota-l') {\rm mod} L}.
%     \label{eq:recover erasure}
% \end{equation}
% We see that it suffice to let $m\leq (J-m)$ and all matrix of $\{ \bold{G}_{r}\in \mathbb{F}_2^{m \times (J-m)} \}_{r=1}^M$ have full rank. In this example, though $\wv(l)$ is uniquely determined using any one of $M$ equations in \eqref{eq:recover erasure}, checking if all $M$ equaions give the same $\bold{w}(l)$ reduces PHP in general cases.

% % A noticible point here is that if a path contains an $\na$ in its section $l$, then according to \eqref{eq:parity equation 2}, the next consecutive $M$ sections' parity cannot be calculated. Hence in the worst case we again need to stitch all entries in the lists of section $\{l+1,l+2,\ldots,l+M\}$. In some luckier cases, we may have $l+M > L-1$, or we can fully determine the lost $\wv(l)$ using any one equation of \eqref{eq:recover erasure} in an earlier time.


%
%\sr{still have to check}
%


For the sake of compactness, we present the decoding algorithm through pseudo-code in Alg.~\ref{alg:cap}. 
Therein, $\textbf{checkParity}(\uv)$ simply checks whether the parity bits of all sections of the input $\uv$ are consistent with \eqref{eq:parity equation 3}; thus, it returns $\textbf{False}$ if and only if \eqref{eq:parity equation 3} is violated with all involved sections that are present as explicit bits in $\uv$. 
Hence when a path is of length $\leq M$, it will always be parity-consistent because no section's parity can be checked at all. 
% 
The subroutine $\textbf{checkParityWithRcv}(\uv)$ serves a similar purpose, except for when $\uv$ contains an $\na$, it tries to uniquely determine the lost information bits according to \eqref{eq:parity equation 3} by reverse-engineering. 
This can be done when we choose matrices in $\{\Gv_r\}_{r=1}^M$ that admit a right-inverse.

\begin{algorithm}[H]
\caption{Pseudo code of the LLC decoding algorithm.}
%\sr{still have to check}}
\label{alg:cap}
\begin{algorithmic}[1]
\Require UACE output $\Yv=[\yv(0), \ldots , \yv(L-1)]$ 
\Ensure 
% $M \in [1:L]$; 
$\forall \ l \in [L]$, $|\yv(l)| \leq K$; 
% \bold{G}_{l_1,l_2} $ are full rank and fat.

\Comment Decoding phase $1$

\State $\Lsf^1 \gets \emptyset$; $\widehat{\Wv}^1 \gets \emptyset$
\ForEach{$l \in [L]$}
    \ForEach{$\uv \in (\Lsf^1 \text{ if } \Lsf^1\neq \emptyset \text{ else } \{\emptyset\})$}
        \State $\Lsf^1 \gets \Lsf^1 - \{\uv\}$
        \ForEach{$x(l) \in \yv(l)$}
            \If{\textbf{checkParity}$(\bold{u}. x(l))$}
                \State $\Lsf^1 \gets \Lsf^1 \cup \{\uv.x(l)\}$
            \EndIf
        \EndFor
    \EndFor
\EndFor

\State $\widehat{\Wv}^1 \gets \textbf{extractInfoBits}(\Lsf^1)$

\Comment{Decoding phase $2$}

\State $\Lsf^2 \gets \emptyset$; $\widehat{\Wv}^2 \gets \emptyset$

\ForEach{$x(0)^\times \in \yv(0)$ leads to no element in $\Lsf^1$}
    \State $\Lsf^2(x(0)^\times) \gets \{x(0)^\times \}$
    \ForEach{$l \in \{1,2,\ldots,L-1\}$}
        \ForEach{$\uv \in \Lsf^2(x(0)^\times)$}
            \State $\Lsf^2(x(0)^\times) \gets \Lsf^2(x(0)^\times) - \{\uv\}$
            \If{$\uv \text{ contains no } \na$ }
                \State $\Lsf^2(x(0)^\times) \gets \Lsf^2(x(0)^\times) \cup \{\uv . \na \}$

            \EndIf
            \ForEach{$x(l) \in \yv(l)$}
                \If{$\textbf{checkParityWithRcv}(\uv . x(l))$}
                    \State $\Lsf^2(x(0)^\times) \gets \Lsf^2(x(0)^\times) \cup \{\uv . x(l)\}$
                \EndIf
            \EndFor
        \EndFor
    \EndFor

    \State $\Lsf^2 \gets \Lsf^2 \cup \Lsf^2(x(0)^\times)$
\EndFor

% \ForEach{$\uv \in \Lsf^2$}
%     \State $\Lsf^2 \gets \Lsf^2 - \{\uv \} \text{ if } \textbf{checkParityWithRcv}(\uv) \neq \textbf{True} $
% \EndFor

\State $\widehat{\Wv}^2 \gets \textbf{extractInfoBits}(\Lsf^2)$

\State $\widehat{\Wv} \gets \widehat{\Wv}^1 \cup \widehat{\Wv}^2$

\State \Return $\widehat{\Wv}$

% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf

\end{algorithmic}
\end{algorithm}


==> related_results.tex <==

\section{ Related Results}
\label{sec:Related Results}
In our numerical simulations, we shall compare the performance of the LLC with the tree code from \cite{amalladinne2020coded} and the LDPC code from \cite{amalladinne2021unsourced}.
%
We stress that both of these codes were not originally designed for the UACE model and, as such this comparison offers only limited insight.
 %
These schemes are selected as benchmarks because they are readily applicable to the problem at hand.


%\subsection{Tree code}
%\sr{complete}
%

\noindent
{\bf Tree code (TC):}
The tree code of \cite{amalladinne2020coded} is a binary linear code in which the length of parity bits, $p(l)$, increases by each section. 
%
In decoding, it is assumed that $Y$ in \eqref{eq:channel error} does not contain any erasures but possibly contains additional, untransmitted symbols.
% , as discussed in 
% Sec. \ref{sec:Motivation and Further comments}. 
%
For this reason, the decoding algorithm is substantially equivalent to phase~$1$ in the LLC decoding, with the difference that the number of parity bits increases with the section number, thus allowing for a more efficient pruning of surviving paths. 


%\subsection{Belief Propagation Code}
\noindent
{\bf LDPC:}
Another candidate coding scheme for the UACE is the triadic LDPC code with belief propagation (BP) decoding of \cite{amalladinne2021unsourced}.
%
In this approach, sections are viewed as symbols over a Galois field and they are encoded using a non-binary LDPC code; therein, sections contain either all information bits or all parity bits. 
%
Parity sections are obtained from information sections as in a classic LDPC code. 
%
The FFT method for decoding non-binary LDPC codes is leveraged to efficiently implement message passing between parity sections and information sections.

%
% \begin{figure}
%     \centering
%     \include{figures/ldpc_factor_graph}
%     \caption{\textcolor{blue}{update caption later}}
%     \label{fig:ldpc_factor_graph}
% \end{figure}
%
%\sr{WZ: add the figures from Jamison}


==> simulations.tex <==

\section{Simulation Results}
\label{sec:Simulation Results}
In this section, we study the performance of the LLC on the UACE with hyperparameters tuned to practical applications. 
%
We provide a comparison with the tree code of \cite{amalladinne2020coded} and the LDPC code of \cite{amalladinne2021unsourced}. 
We consider a system with $K$ active users, each having $B=128$ bits of information to transmit. 
%
The corresponding codewords are divided into $L=16$ sub-blocks, each of length $J=16$. 
%\textcolor{red}{
For the tree code, the specific value for $m(l)$ leads to different discriminating power and was chosen carefully after extensive numerical experimentation. 
%to techniques. 
%While for LLC, the value for $m$ is determined by rate only.
%} 
Comparison of the three codes using fixed $K=100$ and varying $p_e \in [0,0.15]$ is shown in Fig.~\ref{fig:llc_vs_tc_vs_ldpc}. Compared to TC and LDPC code, LLC offers a noticeable improvements in terms of greatly decaying the PDP due to phase 2 of decoding, while keeping PHP in a low level. Fig.~\ref{fig:only_llc} shows how LLC itself performs under different $(K,p_e)$ with $K\in [50,150]$.



\begin{enumerate}
    \item canonical performance A/B channel  Pphp/Ppdp 
    \item SIC A/B channel  Pphp/Ppdp     
    \item  A/B channel: pe vs Num user -> info bits fixed, pdp<0.1 (do this for different rates)
    \item fix number of users, fix probability of  erasure, try different code rates, plot Pphp/Ppdp and  show where we want to operate  
    \item effect window size: trade off complexity performance: Pphp/Ppdp 
    \item  illustrate non convex behavioir: for some codes Pphp/Ppdp is not convex
    \item  comparison between LLC/TC/LDPC   
\end{enumerate}

\begin{figure}
  \centering
  \input{figures/llc_vs_tc_vs_ldpc_performance}
  \caption{Empirical $P_{\text{PHP}}$ vs $P_{\text{PDP}}$ for the LLC (with $M=2$), tree code, and LDPC code. Here, $K = 100$, and the $p_e$ associated with each point is labelled on the graph.
  %under fixed $K=100$ and varying $p_e$ labelled beside.
  }
 \label{fig:llc_vs_tc_vs_ldpc}
\end{figure}

\begin{figure}
  \centering
  \input{figures/only_llc_changing_kpe}
  \caption{Empirical $P_{\text{PHP}}$ vs $P_{\text{PDP}}$ of the LLC (with $M=2$) for various values of $K$ and $p_e$. The label associated with each data point indicates the $p_e$. }
 \label{fig:only_llc}
\end{figure}



